The Local Cluster Survey II: Disk-Dominated Cluster Galaxies with Suppressed Star Formation

We investigate the role of dense environments in suppressing star formation by studying $\rm \log_{10}(M_\star/M_\odot) > 9.7$ star-forming galaxies in nine clusters from the Local Cluster Survey ($0.0137 < z < 0.0433$) and a large comparison field sample drawn from the Sloan Digital Sky Survey. We compare the star-formation rate (SFR) versus stellar mass relation as a function of environment and morphology. After carefully controlling for mass, we find that in all environments, the degree of SFR suppression increases with increasing bulge-to-total (B/T) ratio. In addition, the SFRs of cluster and infall galaxies at a fixed mass are more suppressed than their field counterparts at all values of B/T. These results suggest a quenching mechanism that is linked to bulge growth that operates in all environments and an additional mechanism that further reduces the SFRs of galaxies in dense environments. We limit the sample to $B/T < 0.3$ galaxies to control for the trends with morphology and find that the excess population of cluster galaxies with suppressed SFRs persists. We model the timescale associated with the decline of SFRs in dense environments and find that the observed SFRs of the cluster core galaxies are consistent with a range of models including: a mechanism that acts slowly and continuously over a long (2-5 Gyr) timescale, and a more rapid ($<1$ Gyr) quenching event that occurs after a delay period of 1-6 Gyr. Quenching may therefore start immediately after galaxies enter clusters.

==> table1.tex <==
\begin{table*}%[h] 
\centering 
\begin{tabular}{|c|c|c|c|c|c|} 
\hline
Samples &Variable  &\multicolumn{2}{c|}{All $B/T$} &  \multicolumn{2}{c|}{$B/T < 0.3$}\\ 
& & \multicolumn{2}{c|}{KS p value}& \multicolumn{2}{c|}{KS p value} \\ 
& &  no mass match & mass match & no mass match & mass match\\ 
\hline \hline 
LCS Core-Field    & $\log SFR$         & \bf 1.29e-05 & \bf 2.97e-02 & \bf 1.87e-05& \bf 1.16e-02 \\ 
 & $\Delta \log $SFR  & \bf 1.13e-05 & \bf 1.42e-02 & \bf 1.16e-04 & \bf 1.88e-02 \\ 
 & $\log M_\star/M_\odot$    & 5.87e-02 & 8.61e-01 & 5.83e-02 & 9.99e-01  \\ 
 & $B/T$    &\bf 5.24e-03 &\bf 2.73e-03 &\bf 7.57e-03 &\bf 3.74e-01  \\ 
\hline 
LCS Infall-Field  & $\log$ SFR &\bf 8.08e-10 &\bf 1.52e-05 & \bf 3.02e-04 & \bf 2.45e-03\\ 
& $\Delta \log$SFR  & \bf 6.64e-11   & \bf 8.19e-08 & \bf 6.42e-05 & \bf   1.71e-03\\ 
&$\log M_\star/M_\odot$   &  7.24e-01 &  7.60e-01 & 2.47e-01  & 9.99e-01 \\ 
&$B/T$   &  \bf 4.38e-05 & \bf 4.29e-03 & \bf 1.09e-02  & 1.74e-02 \\ 
\hline 
LCS Core-Infall    & $\log$ SFR      & 7.44e-01  & \nodata  & 2.45e-01 &\nodata  \\ 
& $\Delta \log$SFR& 5.58e-01 & \nodata & 3.47e-01  &\nodata  \\ 
& $\log M_\star/M_\odot$ & 2.55e-01  & \nodata & 4.22e-01  &\nodata \\ 
& $B/T$ & 5.23e-01  & \nodata & 1.62e-01  &\nodata \\ 
\hline 
\end{tabular} 
\caption{Summary statistics for SFR, $\Delta$SFR, stellar mass, and $B/T$ comparisons.  Bold text indicates when the two populations differ at the 99.7\% or $\ge 3\sigma$ confidence interval (KS p-value$<$3.0e-03). } 
\label{tab:stats} 
\end{table*} 

